From Global Choreographies to Provably Correct and Efficient Distributed Implementations

We define a method to automatically synthesize provably-correct efficient distributed implementations from high-level global choreographies. A global choreography describes the execution and communication logic between a set of provided processes which are described by their interfaces. The operations at the level of choreographies include multiparty communications, choice, loop, and branching. Choreographies are master-triggered, that is each choreography has one master to trigger its execution. This allows to automatically generate conflict free distributed implementations without controllers. The behavior of the synthesized implementations follows the behavior of choreographies. In addition, the absence of controllers ensures the efficiency of the implementation and reduces the communication needed at runtime. Moreover, we define a translation of the distributed implementations to equivalent Promela versions. The translation allows verifying the distributed system against behavioral properties. We implemented a Java prototype to validate the approach and applied it to automatically synthesize micro-services architectures. We illustrate our method on the automatic synthesis of a verified distributed buying system.

==> correctnessChoreography.tex <==





\section{Verifying correctness of choreographies}



\subsection{Verifying correctness by model checking}

algorithm for generating Kripke structure of choreographies

based on semantics rules of section ??

generates kripke structe in Eshmun, can be model checked and repaiured




\subsection{Compositional verification rules}

to deal woth state explosion in choreographies resulting from use of parallel operator

==> loop.tex <==

\begin{definition}[Loop] 
Consider a system $S$,  we define the $\while$ operator that allows to repeat a session type until a certain condition is met. The condition can be thought of as a boolean variable $g$ that can be either true or false. Then, ($\while$) can be defined as an operator that transforms $S$ into a new system ${\cal S}' = (S', \context') = {\cal S}\semantics[\while(B_i.p_i^{\controlsend_g}) \{\st\}] = \unionst(S^t,S^m, S^f)$, where: (1) ${\cal S}^t = (S^t, \context^t) = {\cal S}\semantics[p_i^{\controlsend_g} \synchronous \{p^{\controlrcv}_j\}_{j \in C} \bullet \st]$, (2) ${\cal S}^f = (S^f, \context^f) = S\semantics[p_i^{\controlsend_n} \synchronous \{p^{\controlrcv}_j\}_{j \in C - \{i\} }]$, and (3) ${\cal S}^m = (\gamma^m(B^m_1,\dots,B^m_n))$ where $\gamma^m = \{\{p_i , \{p_j\}_{j \in C - \{i\}} \}$ and
\begin{align*}
	B^m_k = 
		&\begin{cases}
		  (P^t_k, Q^t_k, T^t_k \cup \{\context^t(B^t_k), p_k, \context(B_k)\})& \forall k \in C\\
			B^t_k & \text{otherwise}
			\end{cases}\\	
			\end{align*}

\end{definition}

\todo{what is p_i?.. Union is not exactly correct, because we only want the context of $S^f$, maybe define a new operation?.. The only purpose of $S^m$ is to add the "go back" transition, could be written better }

==> model-data.tex <==
\section{Semi-Synchronous Component-based Framework}
In this section, we introduce an extension of BIP framework \ldots
Synchronization between the atomic components is defined using the notion of interaction. 

\todo{add text here...}


\todo{discuss the idea of the disadvantage of BIP synchronization model: multiparty with no master requires to build controllers to resolve conflict. Moreover, in practice, a master exists for any interaction. As such, this allows to generate efficient distributed implementations. Question: do we need to restrict the behavior of atomic components by not allowing both send and receive from the same location? To think about it.}

\todo{add note about data, for the sake of simplicity we omitted data from atomic components and only focus on synchronization primitives}

\begin{definition}[Port] 
A port $p$ is defined as a tuple $(\typec, \variables)$, where
\begin{itemize}
\item $\typec \in \{\synchs, \asynchs, \recv\}$, denotes the communication type, synchronous send, asynchronous send, or receive, respectively; 
\item $\variables$ denotes the variable attached to this port. 
\end{itemize}
\end{definition}

We consider a port 
\begin{definition}[Semantics of Port] 
A port $p$ is defined as a tuple $(\typec, \typed)$, where
\end{definition}


\begin{definition}[Atomic Component]
An atomic component $B_i$ is defined as a tuple $(P_i, L_i, X_i, T_i)$, where 
\begin{itemize}
\item $P_i$ is a set of ports; 
\item $L_i$ is a set of locations; 
\item $X_i$ is a set of variables;
\item $T_i \subseteq L_i \times (P_i, \mathtt{\guard}, \mathtt{\function}) \times L_i$ is a set of transitions, where (1) $\guard$ is a Boolean condition over $X_i$: the guard of $\tau$; and (2) $\function$ is a sequence of assignments to variables $X_i$: the computation of $\tau$.
\end{itemize}
\end{definition}

\begin{definition}[Semantics of Atomic Component]
The semantics of atomic component $(P_i, L_i, X_i, T_i)$ is the LTS $(P_i, Q_i, \rightarrow)$, where: (1) 
An atomic component $B_i$ is defined as a tuple $(P_i, Q_i, T_i)$, where (1) $P_i$ is a set of ports; (2) $Q_i$ is a set of states; (3) $T_i \subseteq Q_i \times P_i \times Q_i$ is a set of transitions.   
\end{definition}

In the sequel, we consider a system of $n$ atomic components $\{B_i = (P_i, Q_i, T_i)\}_{i = 1}^{n}$. We define the set ${\cal P} = \cup_{i = 1}^{n} P_i$ (resp. 
${\cal P}^{ss} = \{p \mid p \in {\cal P} \, \wedge \, \mathtt{isSSend}(p)\}$, 
${\cal P}^{as} = \{p \mid p \in {\cal P} \, \wedge \, \mathtt{isASend}(p)\}$, 
${\cal P}^{r} = \{p \mid p \in {\cal P} \, \wedge \, \mathtt{isRecv}(p)\}$)
of all the ports (resp. synchronous send port, asynchronous send ports, receive ports) of the system. Moreover, we denote ${\cal P}_i^{ss}$ (resp. ${\cal P}_i^{as}$, ${\cal P}_i^{r}$) to be the set of all synchronous send (resp., asynchronous send, receive) ports of atomic component $B_i$. We also consider that port $p_i$ belongs to component $i$. 

\begin{definition}[Interaction]
An interaction is $a = (p_i, \{p_j\}_{j \in J})$, where $i \notin J$, is defined by (1) its send port $p_i$ (synchronous or asynchronous) that belongs to the send ports of atomic component $B_i$, i.e., $p_i \in {\cal P}_i^{ss} \cup {\cal P}_i^{as}$; (2) its receive ports $\{p_j\}_{j \in J})$ each of which belong to the receive ports of atomic component $B_j$, i.e., $p_j \in {\cal P}_j^{r}$.
\end{definition}

An interaction $a = (p_i, \{p_j\}_{j \in J})$ is synchronous (resp. asynchronous) interaction iff $\mathtt{isSSend}(p_i)$ (resp. $\mathtt{isASend}(p_i)$).

\begin{definition}[Composite Component] A composite component $B$ is defined by a composition operator parameterized by a set of interactions $\gamma$.  $B = \gamma(B_1, \ldots, B_n$, is a transition system $(Q, \gamma, \rightarrow)$, where $Q = \bigotimes_{i=1}^{n} Q_i$ and $\rightarrow$ is the least set of transitions satisfying the following rules:
\begin{equation}
\frac
{a = (p_i, \{p_j\}_{j \in J}) \in \gamma \quad  \mathtt{isSSend}(p) \quad \forall k \in J \cup \{i\}: q_k \synch[p_k] q'_k \quad \forall k \notin J \cup \{i\}: q_k = q'_k}
{(q_1, \ldots, q_n) \synch[a] (q'_1, \ldots, q'_n)}
\end{equation}

\begin{equation}
\frac
{a = (p_i, \{p_j\}_{j \in J}) \in \gamma \quad  \mathtt{isASend}(p) \quad q_i \synch[p_i] q'_i \quad \forall k \neq i: q_k = q'_k}
{(q_1, \ldots, q_n) \synch[a] (q'_1, \ldots, q'_n) \quad \forall j \in J: p_j.\buffer := p_j.\buffer + 1}
\end{equation}

\begin{equation}
\frac
{a = (p_i, \{p_j\}_{j \in J}) \in \gamma \quad q_j \synch[p_j] q'_j \quad p_j.\buffer > 0 \quad \forall k \neq j: q_k = q'_k}
{(q_1, \ldots, q_n) \synch[a] (q'_1, \ldots, q'_n) \quad p_j.\buffer := p_j.\buffer - 1}
\end{equation}
\end{definition}
